Evolution of a Viscous Protoplanetary Disk with Convectively Unstable Regions. II. Accretion Regimes and Long-Term Dynamics

In this article, we proceed to study convection as a possible factor of episodic accretion in protoplanetary disks. Within the model presented in Article~I, the accretion history is analyzed at different rates and areas of matter inflow from the envelope onto the disk. It is shown that the burst-like regime occurs in a wide range of parameters. The long-term evolution of the disk is also modeled, including the decreasing-with-time matter inflow from the envelope. It is demonstrated that the disk becomes convectively unstable and maintains burst-like accretion onto the star for several million years. Meanwhile, the instability expands to an area of several tens of astronomical units and gradually decreases with time. It is also shown that at early stages in the disk evolution, conditions arise for gravitational instability in the outer parts of the disk and for dust evaporation in the convectively unstable inner regions. The general conclusion of the study is that convection can serve as one of the mechanisms of episodic accretion in protostellar disks, but this conclusion needs to be verified using more consistent hydrodynamic models.

==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%               Macros for TeX/LaTeX documents
%
% Author: Frank C. van den Bosch
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\etal}{{et al.~}}

\newcommand{\kmsmpc}{\>{\rm km}\,{\rm s}^{-1}\,{\rm Mpc}^{-1}}
%\newcommand{\kms}{\>{\rm km}\,{\rm s}^{-1}}
%\newcommand{\pc}{\>{\rm pc}}
\newcommand{\cm}{\>{\rm cm}}
\newcommand{\Mpc}{\>{\rm Mpc}}
\newcommand{\kpc}{\>{\rm kpc}}
\newcommand{\Msun}{\>{\rm M_{\odot}}}
\newcommand{\Lsun}{\>{\rm L_{\odot}}}
\newcommand{\MLsun}{\>({\rm M}/{\rm L})_{\odot}}
\newcommand{\Mbh}{M_{\bullet}}
\newcommand{\Vrot}{V_{\rm rot}}
\newcommand{\mtol}{\>{\rm (M/L)_{\odot}}}
\newcommand{\erg}{\>{\rm erg}}
\newcommand{\kpch}{\>{h^{-1}{\rm kpc}}}
\newcommand{\mpch}{\>h^{-1}{\rm {Mpc}}}
\newcommand{\yr}{\>{\rm yr}}
\newcommand{\yrs}{\>{\rm yrs}}
\newcommand{\Msunh}{\>h^{-1}\rm M_\odot}
\newcommand{\Lsunh}{\>h^{-2}\rm L_\odot}
\newcommand{\calN}{{\cal N}}
\newcommand{\wcalN}{\tilde{{\cal N}}}
\newcommand{\walpha}{\tilde{\alpha}}
\newcommand{\wLstar}{\tilde{L}^{*}}
\newcommand{\hxi}{\hat{\xi}}
\newcommand{\lamA}{${\Lambda}30/90 \, $}
\newcommand{\lamC}{${\Lambda}25/75 \, $}
\newcommand{\lamD}{${\Lambda}20/65 \, $}
\newcommand{\lamB}{${\Lambda}30/65 \, $}
\newcommand{\reference}{\bibitem}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\vcir}{V_{\rm c}}
\newcommand{\vh}{V_{\rm c}}
\newcommand{\Obaryon}{{\Omega_{\rm B,0}}}
\newcommand{\Kdegree}{\>{\rm K}}
\newcommand{\keV}{\>{\rm keV}}
\newcommand{\vhalo}{V_{\rm c}}
\newcommand{\Tvir}{T_{\rm vir}}
\newcommand{\rmd}{{\rm d}}
\newcommand{\vesc}{V_{\rm esc}}
\newcommand{\Lya}{{\rm Ly}\alpha}
\newcommand{\msunh}{\>h^{-1}\rm M_\odot}
\newcommand{\Lsunhh}{\,h^{-2}\rm L_\odot}
\newcommand{\Msunhh}{\,h^{-2}\rm M_\odot}

%%% 
\newcommand{\lcen}{L}
\newcommand{\msc}{M_{\rm *c}}
\newcommand{\pc}{Q}
\newcommand{\pten}{Q_{\rm 10}}
\newcommand{\lc}{\lcen}
\newcommand{\avg}[1]{\langle #1 \rangle}
\newcommand{\avglogm}{\avg{\log M}(\lcen)}
\newcommand{\avglogmsq}{\avg{(\log M)^2}(L_c)}
\newcommand{\avgloglc}{\avg{\log \lcen}(M)}
\newcommand{\siglogm}{\sigma_{\log M}(\lcen)}
\newcommand{\ploglcm}{P(\log \lcen|M)}
\newcommand{\plogmlc}{P(\log M|\lcen)}
\newcommand{\drm}{{\rm d}}
\newcommand{\pdv}{{P (\Delta V)}}
\newcommand{\dv}{{\Delta V}}
% \newcommand{\sigcen}{\sigma_{\rm cen}}
\newcommand{\siglcen}{\sigma_{\log L}}
\newcommand{\sigcenm}{\sigma_{\log M_*}}
\newcommand{\sigmscen}{\sigma_{\log M_*}}
\newcommand{\sigp}{\sigma_{\log Q}}
\newcommand{\sigcenp}{\sigma_{\log Q}}
\newcommand{\sigsw}{\sigma_{\rm sw}}
\newcommand{\sighw}{\sigma_{\rm hw}}
\newcommand{\sigsat}{\sigma_{\rm sat}}
\newcommand{\avgsigsatsq}{\avg{\sigsat^2}}
\newcommand{\avnsat}{\avg{N_{\rm s}}}
\newcommand{\avnsatm}{\avnsat(M)}
\newcommand{\philcm}{\Phi_{\rm c}(L|M)}
\newcommand{\philsm}{\Phi_{\rm s}(L|M)}
\newcommand{\plcm}{P(\lcen|M)}
\newcommand{\pmscm}{P(\msc|M)}
\newcommand{\pmlc}{P(M|\lcen)}
\newcommand{\pmpc}{P(M|\pc)}
\newcommand{\ppcm}{P(\pc|M)}
\newcommand{\sigav}{\sigma_{\rm av}}
%special
\newcommand{\fr}{f_{\rm r}}
\newcommand{\fb}{f_{\rm b}}
\newcommand{\fint}{f_{\rm int}}
\newcommand{\sigr}{\sigma_{\rm r}}
\newcommand{\sigb}{\sigma_{\rm b}}
\newcommand{\Mr}{M_{\rm r}}
\newcommand{\Mb}{M_{\rm b}}
\newcommand{\Rh}{R_{\rm h}}
\newcommand{\Rs}{R_{\rm s}}
\newcommand{\dvh}{(\dv)_{\rm h}}
\newcommand{\dvs}{(\dv)_{\rm s}}
\newcommand{\Sset}{\hat{S}}
%%%%% less than approximate and all that

\def\gtsima{$\; \buildrel > \over \sim \;$}
\def\ltsima{$\; \buildrel < \over \sim \;$}
\def\prosima{$\; \buildrel \propto \over \sim \;$}
\def\gsim{\lower.7ex\hbox{\gtsima}}
\def\lsim{\lower.7ex\hbox{\ltsima}}
\def\simgt{\lower.7ex\hbox{\gtsima}}
\def\simlt{\lower.7ex\hbox{\ltsima}}
\def\simpr{\lower.7ex\hbox{\prosima}}
\def\la{\lsim}
\def\ga{\gsim}
\def\lta{\la}
\def\gta{\ga}

%%%%%% Useful for editing drafts

\newcommand{\XXX}[2]{{\sf #1}}
\newcommand{\QQQ}[1]{{\sc $<$#1$>$}}

%To return to the original version, comment the previous two lines and
%uncomment the next two lines 

%\newcommand{\XXX}[2]{#2}
%\newcommand{\QQQ}[1]{}

%%%%%% Useful for bibliography

\newcommand{\apj}{ApJ}
\newcommand{\apjl}{ApJL}
\newcommand{\apjs}{ApJS}
\newcommand{\aj}{AJ}
\newcommand{\mnras}{MNRAS}
\newcommand{\aap}{A\&A}
\newcommand{\aaps}{A\&AS}
\newcommand{\araa}{ARA\&A}
\newcommand{\nat}{Nature}
\newcommand{\pasp}{PASP}

%%%%%% Useful measures of length for use with psfig

\newdimen\hssize
\hssize=8.4truecm
\newdimen\hdsize
\hdsize=17.7truecm

%%%%%%

\def\fn#1{$^{\ref{#1}}$}
\def\fit#1{\footnotesize \it #1 }
	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

